Performance of 802.11be Wi-Fi 7 with Multi-Link Operation on AR Applications

Since its first release in the late 1990s, Wi-Fi has been updated to keep up with evolving user needs. Recently, Wi-Fi and other radio access technologies have been pushed to their edge when serving Augmented Reality (AR) applications. AR applications require high throughput, low latency, and high reliability to ensure a high-quality user experience. The 802.11be amendment, which will be marketed as Wi-Fi 7, introduces several features that aim to enhance its capabilities to support challenging applications like AR. One of the main features introduced in this amendment is Multi-Link Operation (MLO) which allows nodes to transmit and receive over multiple links concurrently. When using MLO, traffic is distributed among links using an implementation-specific traffic-to-link allocation policy. This paper aims to evaluate the performance of MLO, using different policies, in serving AR applications compared to Single-Link (SL). Experimental simulations using an event-based Wi-Fi simulator have been conducted. Our results show the general superiority of MLO when serving AR applications. MLO achieves lower latency and serves a higher number of AR users compared to SL with the same frequency resources. In addition, increasing the number of links can improve the performance of MLO. Regarding traffic-to-link allocation policies, we found that policies can be more susceptible to channel blocking, resulting in possible performance degradation.

==> acronyms.tex <==
\setabbreviationstyle[acronym]{long-short}
% The form of the entries in this file is \newacronym{label}{acronym}{phrase}
%                                      or \newacronym[options]{label}{acronym}{phrase}
% see "User Manual for glossaries.sty" for the  details about the options, one example is shown below
% note the specification of the long form plural in the line below
%\newacronym[longplural={Debugging Information Entities}]{DIE}{DIE}{Debugging Information Entity}
%
% The following example also uses options
%\newacronym[plural={OSes}, firstplural={operating systems (OSes)}]{OS}{OS}{operating system}

% note the use of a non-breaking dash in long text for the following acronym
%\newacronym{IQL}{IQL}{Independent Q‑Learning}

\newacronym{KTH}{KTH}{KTH Royal Institute of Technology}

\newacronym{LAN}{LAN}{Local Area Network}
% note the use of a non-breaking dash in the following acronym
%\newacronym{WiFi}{Wi-Fi}{Wireless Fidelity}

\newacronym{WLAN}{WLAN}{Wireless Local Area Network}
\newacronym{XR}{XR}{Extended Reality}
\newacronym{SDG}{SDG}{Sustainable Development Goal}
\newacronym{VR}{VR}{Virtual Reality}
\newacronym{AR}{AR}{Augmented Reality}
\newacronym{MR}{MR}{Mixed Reality}
\newacronym{MLO}{MLO}{Multi-Link Operation}

\newacronym{AP}{AP}{Access Point}
\newacronym{STA}{STA}{Station}

\newacronym{KPI}{KPI}{Key Performance Indicator}


\newacronym{SISO}{SISO}{Single Input Single Output}
\newacronym{MAC}{MAC}{Medium Access Control}
\newacronym{PHY}{PHY}{Physical}
\newacronym{QoS}{QoS}{Quality of Service}


\newacronym{RTS}{RTS}{Ready To Send}
\newacronym{CTS}{CTS}{Clear To Send}
\newacronym{OFDMA}{OFDMA}{Orthogonal Frequency-Division Multiple Access}
\newacronym{SUMIMO}{SU-MIMO}{Single-User Multiple-Input  Multiple-Output}
\newacronym{MUMIMO}{MU-MIMO}{Multiple-User Multiple-Input  Multiple-Output}
\newacronym{MIMO}{MIMO}{Multiple-Input Multiple-Output}
\newacronym{MPDU}{MPDU}{MAC Protocol Data Unit}
\newacronym{PPDU}{PPDU}{Physical Protocol Data Unit}
\newacronym{AMPDU}{AMPDU}{Aggregated MAC Protocol Data Unit}
\newacronym{AMSDU}{AMSDU}{Aggregated MAC Service Data Unit}
\newacronym{3GPP}{3GPP}{3rd Generation Partnership Project}
\newacronym{DL}{DL}{Downlink}
\newacronym{UL}{UL}{Uplink}
 
\newacronym{CSMACA}{CSMA/CA}{Carrier Sense Multiple Access with Collision Avoidance}
\newacronym{BO}{BO}{backoff counter}
\newacronym{DCF}{DCF}{Distributed Coordination Function}

\newacronym{DIFS}{DIFS}{\gls{DCF} Inter-Frame Spacing}

\newacronym{BEB}{BEB}{Binary Exponential Backoff}
\newacronym{MLD}{MLD}{Multi-Link Device}
\newacronym{LLC}{LLC}{Logical Link Control}
\newacronym{TG}{TG}{Task Group}
\newacronym{NSTR}{N-STR}{Non-Simultaneous Transmit and Receive}
\newacronym{STR}{STR}{ Simultaneous Transmit and Receive}
\newacronym{RV}{RV}{Reality-Virtuality}
\newacronym{F}{F}{Frame rate}
\newacronym{R}{R}{Data Rate}
\newacronym{PDB}{PDB}{Packet Delay Budget}
\newacronym{M}{M}{Mean}
\newacronym{STD}{STD}{Standard Deviation}
\newacronym{ACK}{ACK}{ACKnowledgment}

\newacronym{MCS}{MCS}{Modulation and Coding Scheme}

\newacronym{CCDF}{CCDF}{Complementary Cumulative Distribution Function}

\newacronym{CDF}{CDF}{Cumulative Distribution Function}
\newacronym{SL}{SL}{Single-Link}
\newacronym{RAT}{RAT}{Radio Access Technology}
\newacronym{RTT}{RTT}{Round-Trip Time}
\newacronym{IEEE}{IEEE}{Institute of Electrical and Electronics Engineers}
\newacronym{CBR}{CBR}{Constant Bit Rate}
\newacronym{SAP}{SAP}{Simultaneous-Access Policy}
\newacronym{AGV}{AGV}{Automatic Guided Vehicle}
